Responsibility Analysis by Abstract Interpretation

Given a behavior of interest in the program, statically determining the corresponding responsible entity is a task of critical importance, especially in program security. Classical static analysis techniques (e.g. dependency analysis, taint analysis, slicing, etc.) assist programmers in narrowing down the scope of responsibility, but none of them can explicitly identify the responsible entity. Meanwhile, the causality analysis is generally not pertinent for analyzing programs, and the structural equations model (SEM) of actual causality misses some information inherent in programs, making its analysis on programs imprecise. In this paper, a novel definition of responsibility based on the abstraction of event trace semantics is proposed, which can be applied in program security and other scientific fields. Briefly speaking, an entity ER is responsible for behavior B, if and only if ER is free to choose its input value, and such a choice is the first one that ensures the occurrence of B in the forthcoming execution. Compared to current analysis methods, the responsibility analysis is more precise. In addition, our definition of responsibility takes into account the cognizance of the observer, which, to the best of our knowledge, is a new innovative idea in program analysis.

==> various-definitions.tex <==
% !TEX root = ./responsibility.tex
\section{Refined Definitions of Responsibility\label{sec:variousdefinitions}}

The simple definition of responsibility (\ref{eq:alpharesponsibility}) proposed in subsection \ref{subsec:simple-definition} is implicitly based on a rule that ``for any property $\behavior$ of interest in the system, the earliest event which guarantees the occurrence of $\behavior$ shall be responsible for $\behavior$''. If the objective of the responsibility analysis is to find all potential causes of $\behavior$ before they really occur, and further amend them to prevent $\behavior$, then this simple definition is well-suited. However, if the objective is to investigate the actual cause of $\behavior$ afterwards in some specific trace, then such a definition of responsibility may be inadequate. The reason is that, in a given trace, there may be more than one events that guarantee the occurrence of $\behavior$, and the earliest one may not be the actual one. 

To solve this problem, this section proposes definitions of responsibility that adopt the \textit{counterfactual rule}: ``if the event had not happened, the behavior $\behavior$ of interest would not occur'', or more precisely, ``an event is responsible for a behavior $\behavior$, if and only if, whether this event happens or not can solely decide the occurrence of $\behavior$''. Furthermore, it is noticed that in some scenarios the responsibility of an event is decided by its consequences (future), while in some other scenarios it depends only on its circumstance (history). Thus, by abstracting the history or future, a lattice of responsibility definitions can be built up. We have to admit that there does no exist a single definition of responsibility that could perfectly handle every scenario, since even in the philosophy of science literature there is a protracted controversy concerning the meaning of responsibility, or say ``cause and effect'' (see for example \cite{Frankel1976} discussing the work of Rom Harr{\'e}). Nevertheless, we believe that, for every scenario, there must exist a satisfactory definition of responsibility in the lattice, dealing with the scenario  and meeting the user's expectation of ``cause and effect''.

\subsection{Counterfactual Definitions of Responsibility}
% https://plato.stanford.edu/entries/causation-counterfactual/

Recall the simple definition of responsibility. In a maximal trace $\tracehistory\traceresponsible\tracefuture$, $\traceresponsible$ is said to responsible for a property $\behavior$, if and only if the occurrence of $\traceresponsible$ after the history $\tracehistory$ can guarantee $\behavior$ in the future execution. However, such a definition does not guarantee that ``if $\traceresponsible$ had not occurred, $\behavior$ would not hold in the future execution'', which is exactly the core of classic causality based on counterfactuals in \cite[Section VII]{Hume-1748}. For example, consider the disjunctive scenario of forest fire, in a trace such that both $A$ and $B$ drop a light match, $A$ is determined to be responsible for burning the forest by our definition, since he guarantees the property ``burning the forest''. But if $A$ does not drop a light match, this cannot prevent ``burning the forest'' in the future. Thus, the definition of responsibility in (\ref{eq:alpharesponsibility}) is not counterfactual, i.e.~related to what has not happened.

We propose a strictly counterfactual responsibility abstraction $\alpharesponsibilitySC{\monitorsymbol\sqb{\observer}}{\maximalsemantics{}}{}$ by reusing the monitor function $\monitor{}{\observer}{}$.
In this new definition, an event $\traceresponsible$ is responsible for some property $\behavior$ in the trace $\tracehistory\traceresponsible\tracefuture$, if not only $\traceresponsible$ guarantees property $\behavior$ (i.e. $\behavior\in\monitor{}{\observer}{\prefixes{\tracehistory\traceresponsible}}\backslash\monitor{}{\observer}{\prefixes{\tracehistory}}$), but, moreover, there exists another event $\traceresponsible'$ such that a property $\behavior'$, which is $\sqsubseteq$-incomparable with $\behavior$ in the lattice $\latticeofprefixproperties$of prefix trace properties, can be immediately guaranteed after replacing $\traceresponsible$ with $\traceresponsible'$ (i.e. $\behavior'\in\monitor{}{\observer}{\prefixes{\tracehistory\traceresponsible'}}$. In addition, by lemma \ref{lemma:monitor-incomparable-property}, we know that $\behavior$ cannot hold in any trace whose prefix is $\tracehistory\traceresponsible'$. That is to say, $\tracehistory\traceresponsible$ guarantees $\behavior$, while $\tracehistory\traceresponsible'$ guarantees $\behavior'$, which further prevents $\behavior$. Thus, by the counterfactual reasoning, $\traceresponsible$ is responsible for $\behavior$. In the particular case of a lattice of four prefix trace properties like in Fig. \ref{fig:prefix-lattice-program-error}, the incomparable property $\behavior'$ can only be the negation of $\behavior$. For example, if $\behavior$ represents \textsf{YES}, then $\behavior'$ must represents \textsf{NO}.

\medskip

\begin{mdframed}[nobreak,frametitle={\colorbox{white}{\normalfont\textit{Strictly counterfactual responsibility abstraction} $\alpharesponsibilitySC{}{}{}$}},frametitleaboveskip=-7pt]
\abovedisplayskip-5pt%
\begin{eqntabular}[fl]{@{}l}
% strictly counterfactual
\alpharesponsibilitySC{\monitorsymbol\sqb{\observer}}{\maximalsemantics{}}{} \in \wp(\setofalltraces)\mapsto\wp(\setofalltraces\times\setofalltraces\times\setofalltraces\times\wp(\setofalltraces)) \nonumber
\\
\alpharesponsibilitySC{\monitorsymbol\sqb{\observer}}{\maximalsemantics{}}{\traceproperty}\triangleq \{\quadruple{\tracehistory}{\traceresponsible}{\tracefuture}{\behavior}\mid\nonumber
\\
\qquad\quad{}\tracehistory\traceresponsible\tracefuture\in\traceproperty\cap\maximalsemantics{}\wedge|\traceresponsible|=1\nonumber
\\
\qquad{}\wedge\behavior\in\monitor{}{\observer}{\prefixes{\tracehistory\traceresponsible}}\backslash\monitor{}{\observer}{\prefixes{\tracehistory}} \nonumber
\\
\qquad{}\wedge\exists\traceresponsible'\in\setofalltraces.\;|\traceresponsible'|=1\nonumber
\\
\qquad{}\wedge\exists\behavior'\in\monitor{}{\observer}{\prefixes{\tracehistory\traceresponsible'}}.\;\behavior\not\sqsubseteq\behavior'\wedge\behavior'\not\sqsubseteq\behavior\} \nonumber
\end{eqntabular}
\end{mdframed}

\medskip

Furthermore, instead of requiring that an incomparable property $\behavior'$ is guaranteed immediately after replacing $\traceresponsible$ with $\traceresponsible'$, we can define another counterfactual responsibility abstraction $\alpharesponsibilityC{\monitorsymbol\sqb{\observer}}{\maximalsemantics{}}{}$ by loosening the requirements, such that $\behavior'$ may be guaranteed after $\traceresponsible'$ and part of future $\tracefuture'\isprefix\tracefuture$.  Hence, we have $\behavior\in\monitor{}{\observer}{\prefixes{\tracehistory\traceresponsible\tracefuture'}}$, and $\behavior'\in\monitor{}{\observer}{\prefixes{\tracehistory\traceresponsible'\tracefuture'}}$ which further prevents $\behavior$ to hold in any trace larger than or equal to $\tracehistory\traceresponsible'\tracefuture'$. The only difference between $\tracehistory\traceresponsible\tracefuture'$ and $\tracehistory\traceresponsible'\tracefuture'$ is $\traceresponsible$, thus $\traceresponsible$ must be responsible for $\behavior$. In addition, it is obvious that $\alpharesponsibilitySC{}{}{}$ is a special case of $\alpharesponsibilityC{}{}{}$ by requiring $\tracefuture'$ to be $\emptytrace$.

\medskip

\begin{mdframed}[nobreak,frametitle={\colorbox{white}{\normalfont\textit{Counterfactual responsibility abstraction} $\alpharesponsibilityC{}{}{}$}},frametitleaboveskip=-7pt]
\abovedisplayskip-6pt\arraycolsep0.75\arraycolsep
\begin{eqntabular}[fl]{@{}l}
% counterfactual
\alpharesponsibilityC{\monitorsymbol\sqb{\observer}}{\maximalsemantics{}}{} \in \wp(\setofalltraces)\mapsto\wp(\setofalltraces\times\setofalltraces\times\setofalltraces\times\wp(\setofalltraces)) \nonumber
\\
\alpharesponsibilityC{\monitorsymbol\sqb{\observer}}{\maximalsemantics{}}{\traceproperty}\triangleq \{\quadruple{\tracehistory}{\traceresponsible}{\tracefuture}{\behavior}\mid\nonumber
\\
\qquad\quad{}\tracehistory\traceresponsible\tracefuture\in\traceproperty\cap\maximalsemantics{}\wedge|\traceresponsible|=1\nonumber
\\
\qquad{}\wedge\behavior\in\monitor{}{\observer}{\prefixes{\tracehistory\traceresponsible}}\backslash\monitor{}{\observer}{\prefixes{\tracehistory}} \nonumber
\\
\qquad{}\wedge\exists\traceresponsible', \tracefuture', \tracefuture''\in\setofalltraces.\;|\traceresponsible'|=1\wedge\tracefuture=\tracefuture'\tracefuture''\nonumber
\\
\qquad{}\wedge\exists\behavior'\in\monitor{}{\observer}{\prefixes{\tracehistory\traceresponsible'\tracefuture'}}.\;\behavior\not\sqsubseteq\behavior'\wedge\behavior'\not\sqsubseteq\behavior\} \nonumber
\end{eqntabular}
\end{mdframed}

\medskip

After comparing the definitions of $\alpharesponsibility{}{}{}$, $\alpharesponsibilityC{}{}{}$ and $\alpharesponsibilitySC{}{}{}$, we know $\alpharesponsibilityC{\monitorsymbol\sqb{\observer}}{\maximalsemantics{}}{\traceproperty}$ is an abstraction of $\alpharesponsibility{\monitorsymbol\sqb{\observer}}{\maximalsemantics{}}{\traceproperty}$ (i.e. $\alpharesponsibilityC{\monitorsymbol\sqb{\observer}}{\maximalsemantics{}}{\traceproperty}=\alphaC{\monitorsymbol\sqb{\observer}}{}\circ\alpharesponsibility{\monitorsymbol\sqb{\observer}}{\maximalsemantics{}}{\traceproperty}$), and $\alpharesponsibilitySC{\monitorsymbol\sqb{\observer}}{\maximalsemantics{}}{\traceproperty}$ is an abstraction of $\alpharesponsibilityC{\monitorsymbol\sqb{\observer}}{\maximalsemantics{}}{\traceproperty}$ (i.e. $\alpharesponsibilitySC{\monitorsymbol\sqb{\observer}}{\maximalsemantics{}}{\traceproperty}=\alphaSC{\monitorsymbol\sqb{\observer}}{}\circ\alpharesponsibilityC{\monitorsymbol\sqb{\observer}}{\maximalsemantics{}}{\traceproperty}$), where

\bgroup\arraycolsep0.8\arraycolsep\begin{eqntabular}[fl]{@{}l}
% abstraction
\alphaC{\monitorsymbol\sqb{\observer}}{},\alphaSC{\monitorsymbol\sqb{\observer}}{} \in \wp(\setofalltraces{\times\,}\setofalltraces{\times\,}\setofalltraces{\times\,}\wp(\setofalltraces))\nonumber
\\
\qquad\qquad\qquad\qquad\quad{}\mapsto\wp(\setofalltraces{\times\,}\setofalltraces{\times\,}\setofalltraces\times\wp(\setofalltraces)) \nonumber
\\
\alphaC{\monitorsymbol\sqb{\observer}}{\mathcal{R}}\triangleq \{\quadruple{\tracehistory}{\traceresponsible}{\tracefuture}{\behavior}\in\mathcal{R}\mid\nonumber
\\
\qquad\quad{}\exists\traceresponsible', \tracefuture', \tracefuture''\in\setofalltraces.|\traceresponsible'|=1\wedge\tracefuture=\tracefuture'\tracefuture''\nonumber
\\
\qquad{}\wedge\exists\behavior'\in\monitor{}{\observer}{\prefixes{\tracehistory\traceresponsible'\tracefuture'}}.\;\behavior\not\sqsubseteq\behavior'\wedge\behavior'\not\sqsubseteq\behavior\}\nonumber
\\
\alphaSC{\monitorsymbol\sqb{\observer}}{\mathcal{R}}\triangleq \{\quadruple{\tracehistory}{\traceresponsible}{\tracefuture}{\behavior}\in\mathcal{R}\mid\exists\traceresponsible'\in\setofalltraces.\;|\traceresponsible'|=1\nonumber
\\
\qquad{}\wedge\exists\behavior'\in\monitor{}{\observer}{\prefixes{\tracehistory\traceresponsible'}}.\;\behavior\not\sqsubseteq\behavior'\wedge\behavior'\not\sqsubseteq\behavior\}\nonumber
\end{eqntabular}\egroup

\begin{lemma}\label{lemma:counterfactual-definitions}
$\forall\traceproperty\in\wp(\setofalltraces)$, $\alpharesponsibilitySC{\monitorsymbol\sqb{\observer}}{\maximalsemantics{}}{\traceproperty}\subseteq\alpharesponsibilityC{\monitorsymbol\sqb{\observer}}{\maximalsemantics{}}{\traceproperty}\subseteq\alpharesponsibility{\monitorsymbol\sqb{\observer}}{\maximalsemantics{}}{\traceproperty}$.
\end{lemma}

\begin{example}[House Fire]\label{ex:House-Fire}Consider a revised example originally from \cite{Wright-Causation1988}: one arsonist named $A$ starts a fire east of a house, and then another arsonist named $B$ starts a fire west of this house. The two fires are advancing toward the house, and similar to the disjunctive scenario of forest fire example, each fire is independently sufficient to burn down the house if it reaches the house. Suppose $B$ is closer to the house, and the house is burnt down by the west side fire. 
\end{example}%finishing later with \qed
For the sake of clarity, this real life situation of the house fire can be equivalently transformed into a program in Fig. \ref{fig:house-fire-program}, in which the variable \texttt{A} and \texttt{B} represents the arsonists (value 0 stands for fire, and 1 stands for no fire), \texttt{D} represents the direction of reaching fire (2 stands for the direction of \texttt{B} (west side), 1 stands for the direction of \texttt{A} (east side), and 0 means no fire reaches), and \texttt{H} represents the house (value 0 and later the division by zero means that the house is destroyed, while value 1 means the house is intact). It is necessary to have the variable \texttt{D} indicating the direction, otherwise in the case where both \texttt{A} and \texttt{B} start a fire, it is impossible to distinguish whether the reaching fire is from \texttt{A} or \texttt{B}, no matter we use the event trace model or structural equations model.

\medskip

\begin{figure}[ht]
\vskip-1em
%\begin{wrapfigure}[11]{l}[0pt]{0.45\textwidth}
\footnotesize\ttfamily\abovedisplayskip0pt\belowdisplayskip-1.75em\raggedright
void foo2() \{\\
\quad  int A, B, D, H;\\
\quad  A = input\_1(); //Input 0 or 1\\
\quad  B = input\_2(); //Input 0 or 1\\
\quad  D = (B==0) ? 2 : ((A==0) ? 1 : 0);\\
\quad  H = (B==0) ? B : ((A==0) ? A : 1);\\
\quad  H= 1 / H; //Division by Zero\\
\quad  return; \}\\
\caption{Program Equivalent to House Fire Example\label{fig:house-fire-program}}
%\end{wrapfigure}
\vskip-0.75em
\end{figure}

\noindent The responsibility analysis starts with building a lattice of prefix trace properties of interest, and it is intuitive to create the lattice $\latticeofprefixproperties$ in Fig. \ref{fig:prefix-lattice1-house-fire} with four elements: the top $\prefixtracepropertytop=\prefixsemantics{}$ means it is uncertain if the house is burnt or not; \texttt{YES} = $\{\trace\in\setofalltraces\mid(\texttt{A=0 B=0}\isprefix\trace)\vee(\texttt{A=0 B=1}\isprefix\trace)\vee(\texttt{A=1 B=0}\isprefix\trace)\}$, i.e. the house is ensured to be destroyed if at least one arsonist starts a fire; \texttt{NO} = $\{\trace\in\setofalltraces\mid\texttt{A=1 B=1}\isprefix\trace\}$, i.e. the house is guaranteed to be intact; $\prefixtracepropertybot=\emptyset$ means the house is both destroyed and intact, which is impossible.

\begin{center}
\begin{figure}[h]
\vskip-1em
\mbox{}\hskip0em
\begin{subfigure}[t]{.45\textwidth}
\centering
\begin{tikzpicture}[scale=1]
\footnotesize
    %\tikzstyle{arrow}=[shorten >=-2pt, shorten <=-2pt]
     \draw (1,0) node[name=BOT] {{$\prefixtracepropertybot$}};
     \draw (0,1) node[name=YES] {{\textsf{YES}}};
     \draw (2,1) node[name=NO] {{\textsf{NO}}};
     \draw (1,2) node[name=TOP] {{$\prefixtracepropertytop$}};

     \draw[semithick] (BOT) -- (YES);
     \draw[semithick] (BOT) -- (NO);
     \draw[semithick] (TOP) -- (YES);
     \draw[semithick] (TOP) -- (NO);

\end{tikzpicture}
\vskip-0.33em
\caption{Lattice without Fire Direction Information\label{fig:prefix-lattice1-house-fire}}
\label{fig:prefix-lattice2-house-fire}
\end{subfigure}
\hfill
% The second subfigure
\begin{subfigure}[t]{.5\textwidth}
\centering
\begin{tikzpicture}[scale=1]
\footnotesize
    %\tikzstyle{arrow}=[shorten >=-2pt, shorten <=-2pt]
     \draw (2,0) node[name=BOT] {{$\prefixtracepropertybot$}};
     \draw (0,1) node[name=YESA] {{\textsf{YES\_A}}};
     \draw (2,1) node[name=YESB] {{\textsf{YES\_B}}};
     \draw (1,1.75) node[name=YES] {{\textsf{YES}}};
     \draw (4,1) node[name=NO] {{\textsf{NO}}};
     \draw (2,2.5) node[name=TOP] {{$\prefixtracepropertytop$}};

     \draw[semithick] (BOT) -- (YESA);
     \draw[semithick] (BOT) -- (YESB);
     \draw[semithick] (BOT) -- (NO);
     \draw[semithick] (YESA) -- (YES);
     \draw[semithick] (YESB) -- (YES);
     \draw[semithick] (YES) -- (TOP);
     \draw[semithick] (NO) -- (TOP);

\end{tikzpicture}
\vskip-0.33em
\caption{Lattice with Fire Direction Information\label{fig:prefix-lattice2-house-fire}}
 \end{subfigure}
\vskip-0.5em
 \caption{Lattice of Prefix Trace Properties of Interest for House Fire Analysis\label{fig:two-lattices-house-fire}}
\end{figure}
\end{center}
\vskip-2.5em

Suppose the cognizance is that of an omniscient observer $\omniscientobserver$, the monitor function $\monitor{}{\omniscientobserver}{}$ can be easily built from $\latticeofprefixproperties$. Assume that we are interested in $\traceproperty$ = \{\texttt{A=0 B=0 D=2 H=0 H=1/0, A=0 B=1 D=1 H=0 H=1/0, A=1 B=0 D=2 H=0 H=1/0}\}, i.e. the three cases that the house is burnt down. By applying the three responsibility abstractions defined above on $\traceproperty$, we get:
\begin{enumerate}[leftmargin=*,label=(\arabic*)]
\item $\alpharesponsibility{\monitorsymbol\sqb{\observer}}{\maximalsemantics{}}{\traceproperty}=\{\quadruple{\emptytrace}{\texttt{A=0}}{\texttt{B=0 D=2 H=0 H=1/0}}{\textsf{YES}}, \quadruple{\emptytrace}{\texttt{A=0}}{\texttt{B=1 D=1 H=0 H=1/0}}{\textsf{YES}}, \quadruple{\texttt{A=1}}{\texttt{B=0}}{\texttt{D=2 H=0 H=1/0}}{\textsf{YES}}\}$. I.e. if both arsonists start a fire, then \texttt{A} is responsible for burning the house; if only one arsonist starts a fire, then that arsonist is responsible.

\item $\alpharesponsibilityC{\monitorsymbol\sqb{\observer}}{\maximalsemantics{}}{\traceproperty}=\{\quadruple{\emptytrace}{\texttt{A=0}}{\texttt{B=1 D=1 H=0 H=1/0}}{\textsf{YES}}, \quadruple{\texttt{A=1}}{\texttt{B=0}}{\texttt{D=2 H=0 H=1/0}}{\textsf{YES}}\}$. I.e. if only one arsonist starts a fire, then that arsonist is responsible; however, in the case both arsonists start a fire, this definition fails to determine the responsibility.

\item $\alpharesponsibilitySC{\monitorsymbol\sqb{\observer}}{\maximalsemantics{}}{\traceproperty}=\{\quadruple{\texttt{A=1}}{\texttt{B=0}}{\texttt{D=2 H=0 H=1/0}}{\textsf{YES}}\}$. I.e. only in the case that \texttt{B} starts a fire while \texttt{A} does not, this definition would find \texttt{B} responsible, since changing the value of \texttt{B} to 1 would immediately prevent the house from burning.
\end{enumerate}
Intuitively, in the case that both \texttt{A} and \texttt{B} start a fire, $B$ should be responsible for destroying the house, but none of the above three definitions of responsibility handles this case well. A possible solution is to revise the lattice $\latticeofprefixproperties$ to Fig. \ref{fig:prefix-lattice2-house-fire}, such that \textsf{YES} is splitted into two properties: \texttt{YES\_A} = $\{\trace\in\setofalltraces\mid\texttt{A=0 B=1}\isprefix\trace\}$ representing the house is burnt and the fire is from direction of \texttt{A}, and \texttt{YES\_B} = $\{\trace\in\setofalltraces\mid(\texttt{A=0 B=0}\isprefix\trace)\vee(\texttt{A=1 B=0}\isprefix\trace)\}$ representing the house if burnt and the fire is from direction of $B$. Using the revised lattice of prefix trace properties of interest, the responsibility analysis can get more reasonable results, e.g. by the simple abstraction $\alpharesponsibility{\monitorsymbol\sqb{\observer}}{\maximalsemantics{}}{}$, if both \texttt{A} and \texttt{B} start a fire, then \texttt{A} is found responsible for \textsf{YES}, and \texttt{B} is found responsible for \textsf{YES\_B}. However, such a method is cheating in some sense, since usually the lattice of prefix trace properties of interest shall be fixed for a given system. To address this problem, more definitions of responsibility are introduced in the following subsection.
\hfill\IEEEQED

\subsection{A Lattice of Definitions of Responsibility}

We notice that, in many scenarios, whether an event $\traceresponsible$ is responsible for some behavior $\behavior$ depends only on its future $\tracefuture$. Consider the house fire example \ref{ex:House-Fire}, the arsonist \texttt{B} should be responsible for burning the house down, if and only if, the house is burnt by a fire coming from the west side (i.e. the future $\tracefuture$ is \texttt{D=2 H=0 H=1/0}), no matter \texttt{A} started a fire or not (i.e. whether the history $\tracehistory$ is \texttt{A=0} or \texttt{A=1} has no effect on determining \texttt{B}'s responsibility). Furthermore, there exist scenarios such that an event $\traceresponsible$ is responsible for some behavior $\behavior$, no matter what the history $\tracehistory$ or the future $\tracefuture$ is. E.g. if we are concerned about the crime of arson instead of burning down the forest, then any person who lit a fire in the forest shall be responsible for committing a crime of arson, regardless of what happened in the past or what will happen in the future. To handle such scenarios, here we introduce new responsibility abstractions $\alpha\{\monitorsymbol\sqb{\observer}\}\sqb{\maximalsemantics{}}{}$ of type

\begin{eqntabular}[fl]{@{}rcl}
\alpha\{\monitorsymbol\sqb{\observer}\}\sqb{\maximalsemantics{}}{} &\in& \wp(\setofalltraces)\mapsto\wp(\setofalltraces\times\setofalltraces\times\setofalltraces\times\wp(\setofalltraces)\times\setofalltraces\times\setofalltraces)\renumber{6-tuple type}
\end{eqntabular}
such that $\alpha\{\monitorsymbol\sqb{\observer}\}\sqb{\maximalsemantics{}}(\traceproperty)$ is a set of tuples $\sextuple{\tracehistory}{\traceresponsible}{\tracefuture}{\behavior}{\tracehistorybar}{\tracefuturebar}$ where $\tracehistory\traceresponsible\tracefuture$ is a maximal trace of interest from $\traceproperty$, $\tracehistorybar\traceresponsible\tracefuturebar$ is another maximal trace (maybe not from $\traceproperty$) that is referred to determine $\traceresponsible$'s responsibility, and $\traceresponsible$ is said to be responsible for $\behavior$ in $\tracehistory\traceresponsible\tracefuture$. The correspondence with the previous 4-tuple type is given by the abstraction
\bgroup\belowdisplayskip0pt\begin{eqntabular}[fl]{@{}l}
\pair{\wp(\setofalltraces{\times\,}\setofalltraces{\times\,}\setofalltraces{\times\,}\wp(\setofalltraces){\,\times\,}\setofalltraces{\times\,}\setofalltraces)}{\subseteq}\galois{\bar{\alpha}}{\bar{\gamma}}\pair{\wp(\setofalltraces{\times\,}\setofalltraces{\times\,}\setofalltraces{\times}\wp(\setofalltraces))}{\subseteq}\nonumber
\end{eqntabular}\egroup
such that
\begin{eqntabular*}{@{}l}
\bar{\alpha}(\mathcal{R})\colsep{\triangleq}\{\quadruple{\tracehistory}{\traceresponsible}{\tracefuture}{\behavior}\mid\exists\tracehistorybar,\tracefuturebar\in\setofalltraces.\;
\sextuple{\tracehistory}{\traceresponsible}{\tracefuture}{\behavior}{\tracehistorybar}{\tracefuturebar}\in\mathcal{R}\}.
\end{eqntabular*}

In addition, two abstractions $\alphaHistory{}$ and $\alphaFuture{}$ on the set of 6-tuples are introduced here, which will be used to define responsibility with or without the history or future in the following.
\bgroup\arraycolsep0.8\arraycolsep\begin{eqntabular}[fl]{@{}rcl}
% abstraction
\alphaHistory{},\alphaFuture{} &\in& \wp(\setofalltraces{\times\,}\setofalltraces{\times\,}\setofalltraces{\times\,}\wp(\setofalltraces){\,\times\,}\setofalltraces{\times\,}\setofalltraces)\mapsto\wp(\setofalltraces{\times\,}\setofalltraces{\times\,}\setofalltraces\times\wp(\setofalltraces){\,\times\,}\setofalltraces{\times\,}\setofalltraces) \nonumber\\
\alphaHistory{\mathcal{R}}&\triangleq& \{\sextuple{\tracehistory}{\traceresponsible}{\tracefuture}{\behavior}{\tracehistorybar}{\tracefuturebar}\in\mathcal{R}\mid\tracehistorybar=\tracehistory\} \renumber{history abstraction}\\
% abstraction
\alphaFuture{\mathcal{R}}&\triangleq& \{\sextuple{\tracehistory}{\traceresponsible}{\tracefuture}{\behavior}{\tracehistorybar}{\tracefuturebar}\in\mathcal{R}\mid\tracefuturebar=\tracefuture\} \renumber{future abstraction}
\end{eqntabular}\egroup

\subsubsection{Simple Responsibility in 6-Tuple Type}
For the simple responsibility $\alpharesponsibility{\monitorsymbol\sqb{\observer}}{\maximalsemantics{}}{}$, four new abstractions in 6-tuple type can be given, where $\tracehistorybar\traceresponsible\tracefuturebar$
is a maximal trace for reference that satisfies all the conditions in the definition of $\alpharesponsibility{\monitorsymbol\sqb{\observer}}{\maximalsemantics{}}{}$, the history is kept if $\tracehistory=\tracehistorybar$, and the future is kept if $\tracefuture=\tracefuturebar$.

\begin{enumerate}[leftmargin=*,label={(\arabic*)}]
\item\label{alpharesponsibilityTop}{\textit{Responsibility without history and future.\quad}} $\alpharesponsibilityTop{\monitorsymbol\sqb{\observer}}{\maximalsemantics{}}{}$ ignores both the history $\tracehistorybar$ and future $\tracefuturebar$, and concludes that $\traceresponsible$ is responsible for $\behavior$ in any trace $\tracehistory\traceresponsible\tracefuture$ that contains $\traceresponsible$;
\begin{eqntabular}[fl]{@{}rcl}
% Ignore both the history and future
%%%\alpharesponsibilityCTop{\monitorsymbol\sqb{\observer}}{\maximalsemantics{}}{} &\in& \wp(\setofalltraces)\mapsto\wp(\setofalltraces\times\setofalltraces\times\setofalltraces\times\wp(\setofalltraces)\times\setofalltraces\times\setofalltraces) \nonumber
%%%\\
\alpharesponsibilityTop{\monitorsymbol\sqb{\observer}}{\maximalsemantics{}}{\traceproperty}&\triangleq&\{\sextuple{\tracehistory}{\traceresponsible}{\tracefuture}{\behavior}{\tracehistorybar}{\tracefuturebar}\mid\tracehistorybar\traceresponsible\tracefuturebar\in\maximalsemantics{}\wedge|\traceresponsible|=1\nonumber
\\
&&\renumber{${}\wedge\behavior\in\monitor{}{\observer}{\prefixes{\tracehistorybar\traceresponsible}}\backslash\monitor{}{\observer}{\prefixes{\tracehistorybar}}\wedge\tracehistory\traceresponsible\tracefuture\in\traceproperty\cap\maximalsemantics{}\}$}
\end{eqntabular}

\item\label{alpharesponsibilityH}{\textit{Responsibility with history only.\quad}} $\alpharesponsibilityH{\monitorsymbol\sqb{\observer}}{\maximalsemantics{}}{}$ keeps only the history $\tracehistorybar$ and ignores the future $\tracefuturebar$, and concludes that $\traceresponsible$ is responsible for $\behavior$ in any trace $\tracehistory\traceresponsible\tracefuture$ such that $\tracehistory=\tracehistorybar$;
\begin{eqntabular}[fl]{@{}rcl}
% Keep only the history
\alpharesponsibilityH{\monitorsymbol\sqb{\observer}}{\maximalsemantics{}}{\traceproperty}&\triangleq&\alphaHistory{}\circ\alpharesponsibilityTop{\monitorsymbol\sqb{\observer}}{\maximalsemantics{}}{\traceproperty}\nonumber\\
&=&
\{\sextuple{\tracehistory}{\traceresponsible}{\tracefuture}{\behavior}{\tracehistorybar}{\tracefuturebar}\mid\tracehistorybar\traceresponsible\tracefuturebar\in\maximalsemantics{}\wedge|\traceresponsible|=1\nonumber
\\
&&\renumber{${}\wedge\behavior\in\monitor{}{\observer}{\prefixes{\tracehistorybar\traceresponsible}}\backslash\monitor{}{\observer}{\prefixes{\tracehistorybar}}\wedge\tracehistory\traceresponsible\tracefuture\in\traceproperty\cap\maximalsemantics{}\;$}
\\
&&\renumber{${}\wedge\tracehistory=\tracehistorybar\}$}
\end{eqntabular}

\item\label{alpharesponsibilityF}{\textit{Responsibility with future only.\quad}} $\alpharesponsibilityF{\monitorsymbol\sqb{\observer}}{\maximalsemantics{}}{}$ keeps only the future $\tracefuturebar$ and ignores the history $\tracehistorybar$, and concludes that $\traceresponsible$ is responsible for $\behavior$ in any trace $\tracehistory\traceresponsible\tracefuture$ such that $\tracefuture=\tracefuturebar$;

\begin{eqntabular}[fl]{@{}rcl}
% Keep only the future
\alpharesponsibilityF{\monitorsymbol\sqb{\observer}}{\maximalsemantics{}}{\traceproperty}&\triangleq&\alphaFuture{}\circ\alpharesponsibilityTop{\monitorsymbol\sqb{\observer}}{\maximalsemantics{}}{\traceproperty}\nonumber\\
&=&
\{\sextuple{\tracehistory}{\traceresponsible}{\tracefuture}{\behavior}{\tracehistorybar}{\tracefuturebar}\mid\tracehistorybar\traceresponsible\tracefuturebar\in\maximalsemantics{}\wedge|\traceresponsible|=1\nonumber
\\
&&\renumber{${}\wedge\behavior\in\monitor{}{\observer}{\prefixes{\tracehistorybar\traceresponsible}}\backslash\monitor{}{\observer}{\prefixes{\tracehistorybar}}\wedge\tracehistory\traceresponsible\tracefuture\in\traceproperty\cap\maximalsemantics{}\;$}
\\
&&\renumber{${}\wedge\tracefuture=\tracefuturebar\}$}
\end{eqntabular}

\item\label{alpharesponsibilityBot}{\textit{Responsibility with history and future.\quad}} $\alpharesponsibilityBot{\monitorsymbol\sqb{\observer}}{\maximalsemantics{}}{}$ keeps both the history $\tracehistorybar$ and the future $\tracefuturebar$, and concludes that $\traceresponsible$ is responsible for $\behavior$ in any trace $\tracehistory\traceresponsible\tracefuture$ such that $\tracehistory=\tracehistorybar$ and $\tracefuture=\tracefuturebar$. It is obvious that such a definition is equivalent to the simple responsibility abstraction $\alpharesponsibility{}{}{}$ in 4-tuple type, i.e. $\alpharesponsibility{\monitorsymbol\sqb{\observer}}{\maximalsemantics{}}{\traceproperty}=\bar{\alpha}\circ\alpharesponsibilityBot{\monitorsymbol\sqb{\observer}}{\maximalsemantics{}}{\traceproperty}$.

\begin{eqntabular}[fl]{@{}rcl}
% Keep both the history and the future
%%%\alpharesponsibilityCBot{\monitorsymbol\sqb{\observer}}{\maximalsemantics{}}{} &\in& \wp(\setofalltraces)\mapsto\wp(\setofalltraces\times\setofalltraces\times\setofalltraces\times\wp(\setofalltraces)\times\setofalltraces\times\setofalltraces) \nonumber
%%%\\
\alpharesponsibilityBot{\monitorsymbol\sqb{\observer}}{\maximalsemantics{}}{\traceproperty}&\triangleq&\alphaFuture{}\circ\alpharesponsibilityH{\monitorsymbol\sqb{\observer}}{\maximalsemantics{}}{\traceproperty}\colsep{=}\alphaHistory{}\circ\alpharesponsibilityF{\monitorsymbol\sqb{\observer}}{\maximalsemantics{}}{\traceproperty}\nonumber\\
&=& \{\sextuple{\tracehistory}{\traceresponsible}{\tracefuture}{\behavior}{\tracehistorybar}{\tracefuturebar}\mid\tracehistorybar\traceresponsible\tracefuturebar\in\maximalsemantics{}\wedge|\traceresponsible|=1\nonumber
\\
&&\renumber{${}\wedge\behavior\in\monitor{}{\observer}{\prefixes{\tracehistorybar\traceresponsible}}\backslash\monitor{}{\observer}{\prefixes{\tracehistorybar}}\wedge\tracehistory\traceresponsible\tracefuture\in\traceproperty\cap\maximalsemantics{}\;$}
\\
&&\renumber{${}\wedge\tracehistory=\tracehistorybar\wedge\tracefuture=\tracefuturebar\}$}
\end{eqntabular}
\end{enumerate}

Moreover, we have $\alpharesponsibilityTop{\monitorsymbol\sqb{\observer}}{\maximalsemantics{}}{\traceproperty}=\alpharesponsibilityH{\monitorsymbol\sqb{\observer}}{\maximalsemantics{}}{\traceproperty}\cup\alpharesponsibilityF{\monitorsymbol\sqb{\observer}}{\maximalsemantics{}}{\traceproperty}$, and $\alpharesponsibilityBot{\monitorsymbol\sqb{\observer}}{\maximalsemantics{}}{\traceproperty}=\alpharesponsibilityH{\monitorsymbol\sqb{\observer}}{\maximalsemantics{}}{\traceproperty}\cap\alpharesponsibilityF{\monitorsymbol\sqb{\observer}}{\maximalsemantics{}}{\traceproperty}$.
\subsubsection{Counterfactual Responsibility in 6-Tuple Type}
Similar to $\alphaC{\monitorsymbol\sqb{\observer}}{}$ and $\alphaSC{\monitorsymbol\sqb{\observer}}{}$ defined before, two abstractions $\alphaCbar{\monitorsymbol\sqb{\observer}}{}$ and $\alphaSCbar{\monitorsymbol\sqb{\observer}}{}$ are introduced to define new abstractions in 6-tuple type for counterfactual responsibility and strictly counterfactual responsibility.

\bgroup\arraycolsep0.8\arraycolsep\begin{eqntabular}[fl]{@{}rcl}
% abstraction
\alphaCbar{\monitorsymbol\sqb{\observer}}{},\alphaSCbar{\monitorsymbol\sqb{\observer}}{} &\in& \wp(\setofalltraces{\times\,}\setofalltraces{\times\,}\setofalltraces{\times\,}\wp(\setofalltraces){\,\times\,}\setofalltraces{\times\,}\setofalltraces)\nonumber\\
&&\renumber{$\mapsto\wp(\setofalltraces{\times\,}\setofalltraces{\times\,}\setofalltraces\times\wp(\setofalltraces){\,\times\,}\setofalltraces{\times\,}\setofalltraces)$}\\
\alphaCbar{\monitorsymbol\sqb{\observer}}{\mathcal{R}}&\triangleq& \{\sextuple{\tracehistory}{\traceresponsible}{\tracefuture}{\behavior}{\tracehistorybar}{\tracefuturebar}\in\mathcal{R}\mid\exists\traceresponsible', \tracefuture', \tracefuture''\in\setofalltraces.\;|\traceresponsible'|=1\nonumber
\\
&&\renumber{${}\wedge\tracefuturebar=\tracefuture'\tracefuture''\wedge\exists\behavior'\in\monitor{}{\observer}{\prefixes{\tracehistorybar\traceresponsible'\tracefuture'}}.\;\behavior\not\sqsubseteq\behavior'\wedge\behavior'\not\sqsubseteq\behavior\} $}
\\
\alphaSCbar{\monitorsymbol\sqb{\observer}}{\mathcal{R}}&\triangleq& \{\sextuple{\tracehistory}{\traceresponsible}{\tracefuture}{\behavior}{\tracehistorybar}{\tracefuturebar}\in\mathcal{R}\mid\exists\traceresponsible'\in\setofalltraces.\;|\traceresponsible'|=1\nonumber
\\
&&\renumber{${}\wedge\exists\behavior'\in\monitor{}{\observer}{\prefixes{\tracehistorybar\traceresponsible'}}.\;\behavior\not\sqsubseteq\behavior'\wedge\behavior'\not\sqsubseteq\behavior\} $}
\end{eqntabular}\egroup

By applying $\alphaCbar{\monitorsymbol\sqb{\observer}}{}$ on simple responsibility in 6-tuple type, four new abstractions for counterfactual responsibility can be gained.

\begin{enumerate}[leftmargin=*,label={(\arabic*)}]
\item\label{alpharesponsibilityCTop}{\textit{Counterfactual responsibility without history and future.\quad}}
\begin{eqntabular}[fl]{@{}rcl}
\alpharesponsibilityCTop{\monitorsymbol\sqb{\observer}}{\maximalsemantics{}}{\traceproperty}&\triangleq& 
\alphaCbar{\monitorsymbol\sqb{\observer}}{}\circ\alpharesponsibilityTop{\monitorsymbol\sqb{\observer}}{\maximalsemantics{}}{\traceproperty}\nonumber\\
&=&\{\sextuple{\tracehistory}{\traceresponsible}{\tracefuture}{\behavior}{\tracehistorybar}{\tracefuturebar}\mid\wedge\tracehistorybar\traceresponsible\tracefuturebar\in\maximalsemantics{}\wedge|\traceresponsible|=1\nonumber
\\
&&\quad{}\wedge\behavior\in\monitor{}{\observer}{\prefixes{\tracehistorybar\traceresponsible}}\backslash\monitor{}{\observer}{\prefixes{\tracehistorybar}}\wedge\tracehistory\traceresponsible\tracefuture\in\traceproperty\cap\maximalsemantics{} \nonumber
\\
&&\renumber{${}\wedge\exists\traceresponsible', \tracefuture', \tracefuture''\in\setofalltraces.\;|\traceresponsible'|=1\wedge\tracefuturebar=\tracefuture'\tracefuture''$}
\\
&&\renumber{${}\wedge\exists\behavior'\in\monitor{}{\observer}{\prefixes{\tracehistorybar\traceresponsible'\tracefuture'}}.\;\behavior\not\sqsubseteq\behavior'\wedge\behavior'\not\sqsubseteq\behavior\}$}
\end{eqntabular}

\item\label{alpharesponsibilityCH}{\textit{Counterfactual responsibility with history only.\quad}}
\begin{eqntabular}[fl]{@{}rcl}
\alpharesponsibilityCH{\monitorsymbol\sqb{\observer}}{\maximalsemantics{}}{\traceproperty}&\triangleq&\alphaCbar{\monitorsymbol\sqb{\observer}}{}\circ\alpharesponsibilityH{\monitorsymbol\sqb{\observer}}{\maximalsemantics{}}{\traceproperty}=\alphaHistory{}\circ\alpharesponsibilityCTop{\monitorsymbol\sqb{\observer}}{\maximalsemantics{}}{\traceproperty}\nonumber\\
&=&
\{\sextuple{\tracehistory}{\traceresponsible}{\tracefuture}{\behavior}{\tracehistorybar}{\tracefuturebar}\mid\wedge\tracehistorybar\traceresponsible\tracefuturebar\in\maximalsemantics{}\wedge|\traceresponsible|=1\nonumber
\\
&&\quad{}\wedge\behavior\in\monitor{}{\observer}{\prefixes{\tracehistorybar\traceresponsible}}\backslash\monitor{}{\observer}{\prefixes{\tracehistorybar}}\wedge\tracehistory\traceresponsible\tracefuture\in\traceproperty\cap\maximalsemantics{} \nonumber
\\
&&\renumber{${}\wedge\tracehistory=\tracehistorybar\wedge\exists\traceresponsible', \tracefuture', \tracefuture''\in\setofalltraces.\;|\traceresponsible'|=1\wedge\tracefuturebar=\tracefuture'\tracefuture''$}
\\
&&\renumber{${}\wedge\exists\behavior'\in\monitor{}{\observer}{\prefixes{\tracehistorybar\traceresponsible'\tracefuture'}}.\;\behavior\not\sqsubseteq\behavior'\wedge\behavior'\not\sqsubseteq\behavior\}$}
\end{eqntabular}

\item\label{alpharesponsibilityCF}{\textit{Counterfactual responsibility with future only.\quad}}

\begin{eqntabular}[fl]{@{}rcl}
\alpharesponsibilityCF{\monitorsymbol\sqb{\observer}}{\maximalsemantics{}}{\traceproperty}&\triangleq&\alphaCbar{\monitorsymbol\sqb{\observer}}{}\circ\alpharesponsibilityF{\monitorsymbol\sqb{\observer}}{\maximalsemantics{}}{\traceproperty}=\alphaFuture{}\circ\alpharesponsibilityCTop{\monitorsymbol\sqb{\observer}}{\maximalsemantics{}}{\traceproperty}\nonumber\\
&=&
\{\sextuple{\tracehistory}{\traceresponsible}{\tracefuture}{\behavior}{\tracehistorybar}{\tracefuturebar}\mid\wedge\tracehistorybar\traceresponsible\tracefuturebar\in\maximalsemantics{}\wedge|\traceresponsible|=1\nonumber
\\
&&\quad{}\wedge\behavior\in\monitor{}{\observer}{\prefixes{\tracehistorybar\traceresponsible}}\backslash\monitor{}{\observer}{\prefixes{\tracehistorybar}}\wedge\tracehistory\traceresponsible\tracefuture\in\traceproperty\cap\maximalsemantics{} \nonumber
\\
&&\renumber{${}\wedge\tracefuture=\tracefuturebar\wedge\exists\traceresponsible', \tracefuture', \tracefuture''\in\setofalltraces.\;|\traceresponsible'|=1\wedge\tracefuturebar=\tracefuture'\tracefuture''$}
\\
&&\renumber{${}\wedge\exists\behavior'\in\monitor{}{\observer}{\prefixes{\tracehistorybar\traceresponsible'\tracefuture'}}.\;\behavior\not\sqsubseteq\behavior'\wedge\behavior'\not\sqsubseteq\behavior\}$}
\end{eqntabular}

\item\label{alpharesponsibilityCBot}{\textit{Counterfactual responsibility with history and future.\quad}} It is obvious that such a definition is equivalent to the counterfactual responsibility abstraction $\alpharesponsibilityC{}{}{}$ in 4-tuple type, i.e. $\alpharesponsibilityC{\monitorsymbol\sqb{\observer}}{\maximalsemantics{}}{\traceproperty}\\=\bar{\alpha}\circ\alpharesponsibilityCBot{\monitorsymbol\sqb{\observer}}{\maximalsemantics{}}{\traceproperty}$.

\begin{eqntabular}[fl]{@{}rcl}
\alpharesponsibilityCBot{\monitorsymbol\sqb{\observer}}{\maximalsemantics{}}{\traceproperty}&\triangleq&\alphaCbar{\monitorsymbol\sqb{\observer}}{}\circ\alpharesponsibilityBot{\monitorsymbol\sqb{\observer}}{\maximalsemantics{}}{\traceproperty}\nonumber
\\
&=&\alphaFuture{}\circ\alpharesponsibilityCH{\monitorsymbol\sqb{\observer}}{\maximalsemantics{}}{\traceproperty}=\alphaHistory{}\circ\alpharesponsibilityCF{\monitorsymbol\sqb{\observer}}{\maximalsemantics{}}{\traceproperty}\nonumber
\\
&=&
\{\sextuple{\tracehistory}{\traceresponsible}{\tracefuture}{\behavior}{\tracehistorybar}{\tracefuturebar}\mid\wedge\tracehistorybar\traceresponsible\tracefuturebar\in\maximalsemantics{}\wedge|\traceresponsible|=1\nonumber
\\
&&\quad{}\wedge\behavior\in\monitor{}{\observer}{\prefixes{\tracehistorybar\traceresponsible}}\backslash\monitor{}{\observer}{\prefixes{\tracehistorybar}}\wedge\tracehistory\traceresponsible\tracefuture\in\traceproperty\cap\maximalsemantics{} \nonumber
\\
&&\renumber{${}\wedge\tracehistory=\tracehistorybar\wedge\tracefuture=\tracefuturebar\wedge\exists\traceresponsible', \tracefuture', \tracefuture''\in\setofalltraces.\;|\traceresponsible'|=1\wedge\tracefuturebar=\tracefuture'\tracefuture''$}
\\
&&\renumber{${}\wedge\exists\behavior'\in\monitor{}{\observer}{\prefixes{\tracehistorybar\traceresponsible'\tracefuture'}}.\;\behavior\not\sqsubseteq\behavior'\wedge\behavior'\not\sqsubseteq\behavior\}$}
\end{eqntabular}
\end{enumerate}

%Observe that $\forall\traceproperty\in\wp(\setofalltraces).\;\alpharesponsibilityCBot{\monitorsymbol\sqb{\observer}}{\maximalsemantics{}}{\traceproperty}\subseteq\alpharesponsibilityCF{\monitorsymbol\sqb{\observer}}{\maximalsemantics{}}{\traceproperty}\wedge\alpharesponsibilityCBot{\monitorsymbol\sqb{\observer}}{\maximalsemantics{}}{\traceproperty}\subseteq\alpharesponsibilityCH{\monitorsymbol\sqb{\observer}}{\maximalsemantics{}}{\traceproperty}\wedge\alpharesponsibilityCF{\monitorsymbol\sqb{\observer}}{\maximalsemantics{}}{\traceproperty}\subseteq\alpharesponsibilityCTop{\monitorsymbol\sqb{\observer}}{\maximalsemantics{}}{\traceproperty}\wedge\alpharesponsibilityCH{\monitorsymbol\sqb{\observer}}{\maximalsemantics{}}{\traceproperty}\subseteq\alpharesponsibilityCTop{\monitorsymbol\sqb{\observer}}{\maximalsemantics{}}{\traceproperty}$. 

In addition, we have $\alpharesponsibilityCTop{\monitorsymbol\sqb{\observer}}{\maximalsemantics{}}{\traceproperty}=\alpharesponsibilityCH{\monitorsymbol\sqb{\observer}}{\maximalsemantics{}}{\traceproperty}\cup\alpharesponsibilityCF{\monitorsymbol\sqb{\observer}}{\maximalsemantics{}}{\traceproperty}$, and $\alpharesponsibilityCBot{\monitorsymbol\sqb{\observer}}{\maximalsemantics{}}{\traceproperty}=\alpharesponsibilityCH{\monitorsymbol\sqb{\observer}}{\maximalsemantics{}}{\traceproperty}\cap\alpharesponsibilityCF{\monitorsymbol\sqb{\observer}}{\maximalsemantics{}}{\traceproperty}$.

\begin{example}[House Fire] Continuing the house fire example, assume we are interested in $\traceproperty$ = \{\texttt{A=0 B=0 D=2 H=0 H=1/0}\}. Considering only the future (consequences), the analysis result by $\alpharesponsibilityCF{\monitorsymbol\sqb{\observer}}{\maximalsemantics{}}{\traceproperty}$ is $\{\sextuple{\texttt{A=0}}{\texttt{B=0}}{\texttt{D=2 H=0 H=1/0}}{\textsf{YES}}{\texttt{A=1}}{\texttt{D=2 H=0 H=1/0}}\}$, i.e. in the case both \texttt{A} and \texttt{B} start a fire, \texttt{B} is responsible for burning the house, which is exactly the desired result.
\end{example}

%\begin{eqntabular}[fl]{@{}L@{}rcl}
%% Ignore both the history and future
%%%%&\alpharesponsibilityTop{\monitorsymbol\sqb{\observer}}{\maximalsemantics{}}{} &\in& \wp(\setofalltraces)\mapsto\wp(\setofalltraces\times\setofalltraces\times\setofalltraces\times\wp(\setofalltraces)\times\setofalltraces\times\setofalltraces) \nonumber
%%%%\\
%\rlap{\textit{Responsibility without history and future.\quad}}\nonumber\\
%&\alpharesponsibilityTop{\monitorsymbol\sqb{\observer}}{\maximalsemantics{}}{\traceproperty}&\triangleq& \bar{\alpha}\sqb{\maximalsemantics{}}(\alpharesponsibility{\monitorsymbol\sqb{\observer}}{\maximalsemantics{}}{})\;\traceproperty\nonumber\\
%&&=&\{\sextuple{\tracehistory}{\traceresponsible}{\tracefuture}{\behavior}{\tracehistorybar}{\tracefuturebar}\mid\tracehistory\traceresponsible\tracefuture\in\traceproperty\cap\maximalsemantics{}\wedge|\traceresponsible|=1\nonumber
%\\
%&&&\qquad\qquad\qquad\quad{}\wedge\tracehistorybar\traceresponsible\tracefuturebar\in\maximalsemantics{} \nonumber
%\\
%&&&\qquad\qquad\qquad\quad{}\wedge\behavior\in\monitor{}{\observer}{\prefixes{\tracehistorybar\traceresponsible}}\backslash\monitor{}{\observer}{\prefixes{\tracehistorybar}}\} \nonumber
%\\
%% Keep only the history
%\rlap{\textit{Responsibility without future.\quad}}\nonumber\\
%%%%&\alpharesponsibilityH{\monitorsymbol\sqb{\observer}}{\maximalsemantics{}}{} &\in& \wp(\setofalltraces)\mapsto\wp(\setofalltraces\times\setofalltraces\times\setofalltraces\times\wp(\setofalltraces)\times\setofalltraces\times\setofalltraces) \nonumber
%%%%\\
%&\alpharesponsibilityH{\monitorsymbol\sqb{\observer}}{\maximalsemantics{}}{\traceproperty}&\triangleq& \alphaHistory{}\circ
%\alpharesponsibilityTop{\monitorsymbol\sqb{\observer}}{\maximalsemantics{}}{\traceproperty}\nonumber\\
%&&=&\{\sextuple{\tracehistory}{\traceresponsible}{\tracefuture}{\behavior}{\tracehistorybar}{\tracefuturebar}\mid\tracehistory\traceresponsible\tracefuture\in\traceproperty\cap\maximalsemantics{}\wedge|\traceresponsible|=1\nonumber
%\\
%&&&\qquad\qquad\qquad\quad{}\wedge\tracehistorybar\traceresponsible\tracefuturebar\in\maximalsemantics{}\wedge\tracehistorybar=\tracehistory \nonumber
%\\
%&&&\qquad\qquad\qquad\quad{}\wedge\behavior\in\monitor{}{\observer}{\prefixes{\tracehistorybar\traceresponsible}}\backslash\monitor{}{\observer}{\prefixes{\tracehistorybar}}\} \nonumber
%\\
%% Keep only the future
%\rlap{\textit{Responsibility without history.\quad}}\nonumber\\
%%%%&\alpharesponsibilityF{\monitorsymbol\sqb{\observer}}{\maximalsemantics{}}{} &\in& \wp(\setofalltraces)\mapsto\wp(\setofalltraces\times\setofalltraces\times\setofalltraces\times\wp(\setofalltraces)\times\setofalltraces\times\setofalltraces) \nonumber
%%%%\\
%&\alpharesponsibilityF{\monitorsymbol\sqb{\observer}}{\maximalsemantics{}}{\traceproperty}&\triangleq& \alphaFuture{}\circ
%\alpharesponsibilityTop{\monitorsymbol\sqb{\observer}}{\maximalsemantics{}}{\traceproperty}\nonumber\\
%&&=&\{\sextuple{\tracehistory}{\traceresponsible}{\tracefuture}{\behavior}{\tracehistorybar}{\tracefuturebar}\mid\tracehistory\traceresponsible\tracefuture\in\traceproperty\cap\maximalsemantics{}\wedge|\traceresponsible|=1\nonumber
%\\
%&&&\qquad\qquad\qquad\quad{}\wedge\tracehistorybar\traceresponsible\tracefuturebar\in\maximalsemantics{}\wedge\tracefuturebar=\tracefuture\nonumber
%\\
%&&&\qquad\qquad\qquad\quad{}\wedge\behavior\in\monitor{}{\observer}{\prefixes{\tracehistorybar\traceresponsible}}\backslash\monitor{}{\observer}{\prefixes{\tracehistorybar}}\} \nonumber
%\\
%% Keep both the history and the future
%\rlap{\textit{Responsibility.\quad}}\nonumber\\
%%%%&\alpharesponsibilityBot{\monitorsymbol\sqb{\observer}}{\maximalsemantics{}}{} &\in& \wp(\setofalltraces)\mapsto\wp(\setofalltraces\times\setofalltraces\times\setofalltraces\times\wp(\setofalltraces)\times\setofalltraces\times\setofalltraces) \nonumber
%%%%\\
%&\alpharesponsibilityBot{\monitorsymbol\sqb{\observer}}{\maximalsemantics{}}{\traceproperty}&\triangleq& \alphaFuture{}\circ\alphaHistory{}\circ
%\alpharesponsibilityTop{\monitorsymbol\sqb{\observer}}{\maximalsemantics{}}{\traceproperty}\nonumber\\
%&&=&\{\sextuple{\tracehistory}{\traceresponsible}{\tracefuture}{\behavior}{\tracehistorybar}{\tracefuturebar}\mid\tracehistory\traceresponsible\tracefuture\in\traceproperty\cap\maximalsemantics{}\wedge|\traceresponsible|=1\nonumber
%\\
%&&&\qquad\qquad\qquad\quad{}\wedge\tracehistorybar\traceresponsible\tracefuturebar\in\maximalsemantics{}\wedge\tracehistorybar=\tracehistory \wedge\tracefuturebar=\tracefuture\nonumber
%\\
%&&&\qquad\qquad\qquad\quad{}\wedge\behavior\in\monitor{}{\observer}{\prefixes{\tracehistorybar\traceresponsible}}\backslash\monitor{}{\observer}{\prefixes{\tracehistorybar}}\} \nonumber
%\end{eqntabular}

\subsubsection{Strictly counterfactual responsibility in 6-Tuple Type}
In the similar way, four new definitions for strictly counterfactual responsibility can be obtained by applying $\alphaSCbar{\monitorsymbol\sqb{\observer}}{}$ on counterfactual responsibility in 6-tuple type (for brevity, the detailed definitions are omitted).

% Strictly Counterfactual
\begin{eqntabular}[fl]{@{}L@{\quad}rcl}
% Ignore both the history and future
\rlap{(1) \textit{Strictly counterfactual responsibility without history and future.\quad}}\nonumber\\
&\alpharesponsibilitySCTop{\monitorsymbol\sqb{\observer}}{\maximalsemantics{}}{\traceproperty}&\triangleq& \alphaSCbar{\monitorsymbol\sqb{\observer}}{}\circ\alpharesponsibilityCTop{\monitorsymbol\sqb{\observer}}{\maximalsemantics{}}{\traceproperty}\nonumber
\\
%&&=&\{\sextuple{\tracehistory}{\traceresponsible}{\tracefuture}{\behavior}{\tracehistorybar}{\tracefuturebar}\mid\tracehistory\traceresponsible\tracefuture\in\traceproperty\cap\maximalsemantics{}\wedge|\traceresponsible|=1\nonumber
%\\
%&&&\qquad\qquad\qquad\quad{}\wedge\tracehistorybar\traceresponsible\tracefuturebar\in\maximalsemantics{} \nonumber
%\\
%&&&\qquad\qquad\qquad\quad{}\wedge\behavior\in\monitor{}{\observer}{\prefixes{\tracehistorybar\traceresponsible}}\backslash\monitor{}{\observer}{\prefixes{\tracehistorybar}} \nonumber
%\\
%&&&\qquad\qquad\qquad\quad{}\wedge\exists\traceresponsible'\in\setofalltraces.\;|\traceresponsible'|=1\nonumber
%\\
%&&&\qquad\qquad\qquad\quad{}\wedge\exists\behavior'\in\monitor{}{\observer}{\prefixes{\tracehistorybar\traceresponsible'}}.\;\behavior\not\sqsubseteq\behavior'\wedge\behavior'\not\sqsubseteq\behavior\} \nonumber
%\\
% Keep only the history
\rlap{(2) \textit{Strictly counterfactual responsibility with history only.\quad}}\nonumber\\
%%%&\alpharesponsibilitySCH{\monitorsymbol\sqb{\observer}}{\maximalsemantics{}}{} &\in& \wp(\setofalltraces)\mapsto\wp(\setofalltraces\times\setofalltraces\times\setofalltraces\times\wp(\setofalltraces)\times\setofalltraces\times\setofalltraces) \nonumber
%%%\\
&\alpharesponsibilitySCH{\monitorsymbol\sqb{\observer}}{\maximalsemantics{}}{\traceproperty}&\triangleq& \alphaSCbar{\monitorsymbol\sqb{\observer}}{}\circ\alpharesponsibilityCH{\monitorsymbol\sqb{\observer}}{\maximalsemantics{}}{\traceproperty}=\alphaHistory{}\circ\alpharesponsibilitySCTop{\monitorsymbol\sqb{\observer}}{\maximalsemantics{}}{\traceproperty}\nonumber
%\\
%&&=&\{\sextuple{\tracehistory}{\traceresponsible}{\tracefuture}{\behavior}{\tracehistorybar}{\tracefuturebar}\mid\tracehistory\traceresponsible\tracefuture\in\traceproperty\cap\maximalsemantics{}\wedge|\traceresponsible|=1\nonumber
%\\
%&&&\qquad\qquad\qquad\quad{}\wedge\tracehistorybar\traceresponsible\tracefuturebar\in\maximalsemantics{}\wedge\tracehistorybar=\tracehistory \nonumber
%\\
%&&&\qquad\qquad\qquad\quad{}\wedge\behavior\in\monitor{}{\observer}{\prefixes{\tracehistorybar\traceresponsible}}\backslash\monitor{}{\observer}{\prefixes{\tracehistorybar}} \nonumber
%\\
%&&&\qquad\qquad\qquad\quad{}\wedge\exists\traceresponsible'\in\setofalltraces.\;|\traceresponsible'|=1\nonumber
%\\
%&&&\qquad\qquad\qquad\quad{}\wedge\exists\behavior'\in\monitor{}{\observer}{\prefixes{\tracehistorybar\traceresponsible'}}.\;\behavior\not\sqsubseteq\behavior'\wedge\behavior'\not\sqsubseteq\behavior\} \nonumber
%\end{eqntabular}
%
%\begin{eqntabular}[fl]{@{}L@{\quad}rcl}
% Keep only the future
\\
\rlap{(3) \textit{Strictly counterfactual responsibility with future only.\quad}}\nonumber\\
&\alpharesponsibilitySCF{\monitorsymbol\sqb{\observer}}{\maximalsemantics{}}{\traceproperty}&\triangleq& \alphaSCbar{\monitorsymbol\sqb{\observer}}{}\circ\alpharesponsibilityCF{\monitorsymbol\sqb{\observer}}{\maximalsemantics{}}{\traceproperty}=\alphaFuture{}\circ\alpharesponsibilitySCTop{\monitorsymbol\sqb{\observer}}{\maximalsemantics{}}{\traceproperty}\nonumber
\\
%&&=&\{\sextuple{\tracehistory}{\traceresponsible}{\tracefuture}{\behavior}{\tracehistorybar}{\tracefuturebar}\mid\tracehistory\traceresponsible\tracefuture\in\traceproperty\cap\maximalsemantics{}\wedge|\traceresponsible|=1\nonumber
%\\
%&&&\qquad\qquad\qquad\quad{}\wedge\tracehistorybar\traceresponsible\tracefuturebar\in\maximalsemantics{}\wedge\tracefuturebar=\tracefuture\nonumber
%\\
%&&&\qquad\qquad\qquad\quad{}\wedge\behavior\in\monitor{}{\observer}{\prefixes{\tracehistorybar\traceresponsible}}\backslash\monitor{}{\observer}{\prefixes{\tracehistorybar}} \nonumber
%\\
%&&&\qquad\qquad\qquad\quad{}\wedge\exists\traceresponsible'\in\setofalltraces.\;|\traceresponsible'|=1\nonumber
%\\
%&&&\qquad\qquad\qquad\quad{}\wedge\exists\behavior'\in\monitor{}{\observer}{\prefixes{\tracehistorybar\traceresponsible'}}.\;\behavior\not\sqsubseteq\behavior'\wedge\behavior'\not\sqsubseteq\behavior\} \nonumber
%\\
% Keep both the history and the future
\rlap{(4) \textit{Strictly counterfactual responsibility with history and future.\quad}}\nonumber\\
%%%&\alpharesponsibilityCBot{\monitorsymbol\sqb{\observer}}{\maximalsemantics{}}{} &\in& \wp(\setofalltraces)\mapsto\wp(\setofalltraces\times\setofalltraces\times\setofalltraces\times\wp(\setofalltraces)\times\setofalltraces\times\setofalltraces) \nonumber
%%%\\
&\alpharesponsibilitySCBot{\monitorsymbol\sqb{\observer}}{\maximalsemantics{}}{\traceproperty}&\triangleq& \alphaSCbar{\monitorsymbol\sqb{\observer}}{}\circ\alpharesponsibilityCBot{\monitorsymbol\sqb{\observer}}{\maximalsemantics{}}{\traceproperty}\nonumber
\\
&&=&\alphaFuture{}\circ\alpharesponsibilitySCH{\monitorsymbol\sqb{\observer}}{\maximalsemantics{}}{\traceproperty}=\alphaHistory{}\circ\alpharesponsibilitySCF{\monitorsymbol\sqb{\observer}}{\maximalsemantics{}}{\traceproperty}\nonumber
%\\
%&&=&\{\sextuple{\tracehistory}{\traceresponsible}{\tracefuture}{\behavior}{\tracehistorybar}{\tracefuturebar}\mid\tracehistory\traceresponsible\tracefuture\in\traceproperty\cap\maximalsemantics{}\wedge|\traceresponsible|=1\nonumber
%\\
%&&&\qquad\qquad\qquad\quad{}\wedge\tracehistorybar\traceresponsible\tracefuturebar\in\maximalsemantics{}\wedge\tracehistorybar=\tracehistory \wedge\tracefuturebar=\tracefuture\nonumber
%\\
%&&&\qquad\qquad\qquad\quad{}\wedge\behavior\in\monitor{}{\observer}{\prefixes{\tracehistorybar\traceresponsible}}\backslash\monitor{}{\observer}{\prefixes{\tracehistorybar}} \nonumber
%\\
%&&&\qquad\qquad\qquad\quad{}\wedge\exists\traceresponsible'\in\setofalltraces.\;|\traceresponsible'|=1\nonumber
%\\
%&&&\qquad\qquad\qquad\quad{}\wedge\exists\behavior'\in\monitor{}{\observer}{\prefixes{\tracehistorybar\traceresponsible'}}.\;\behavior\not\sqsubseteq\behavior'\wedge\behavior'\not\sqsubseteq\behavior\} \nonumber
\end{eqntabular}

Similarly, we have $\alpharesponsibilitySCTop{\monitorsymbol\sqb{\observer}}{\maximalsemantics{}}{\traceproperty}=\alpharesponsibilitySCH{\monitorsymbol\sqb{\observer}}{\maximalsemantics{}}{\traceproperty}\cup\alpharesponsibilitySCF{\monitorsymbol\sqb{\observer}}{\maximalsemantics{}}{\traceproperty}$, and $\alpharesponsibilitySCBot{\monitorsymbol\sqb{\observer}}{\maximalsemantics{}}{\traceproperty}=\alpharesponsibilitySCH{\monitorsymbol\sqb{\observer}}{\maximalsemantics{}}{\traceproperty}\cap\alpharesponsibilitySCF{\monitorsymbol\sqb{\observer}}{\maximalsemantics{}}{\traceproperty}$.

To sum up, for any set $\traceproperty$ of traces of interest, we build a lattice of responsibility analysis results in Fig. \ref{fig:lattice-definitions}, in which the top $\top_R=\setofalltraces\times\setofalltraces\times\setofalltraces\times\wp(\setofalltraces)\times\setofalltraces\times\setofalltraces$ means everyone is responsible, the bottom $\bot_R=\emptyset$ means no one is responsible, and every other element represents applying the corresponding abstraction on $\traceproperty$ (e.g. $\alpharesponsibilityTop{}{}{}$ represents $\alpharesponsibilityTop{\monitorsymbol\sqb{\observer}}{\maximalsemantics{}}{\traceproperty}$).

\begin{figure}[h]
\centering
\vskip-1em
\begin{tikzpicture}[scale=0.35]
\footnotesize
    %\tikzstyle{arrow}=[shorten >=-2pt, shorten <=-2pt]
     \draw (0,2) node[name=alpharesponsibilitySC] {{$\alpharesponsibilitySC{}{}{}$}};
     \draw (0,7) node[name=alpharesponsibilityC] {{$\alpharesponsibilityC{}{}{}$}};
     \draw (0,12) node[name=alpharesponsibility] {{$\alpharesponsibility{}{}{}$}};
     \draw[semithick, line width=1pt,<-] (alpharesponsibilitySC) -- (alpharesponsibilityC) node [midway, above, sloped] (TextNode) {$\alphaSC{}$};
     \draw[semithick, line width=1pt,<-] (alpharesponsibilityC) -- (alpharesponsibility) node [midway, above, sloped] (TextNode) {$\alphaC{}$};
     %
     %
     \draw (10,0) node[name=botR] {{$\bot_R$}};
     \draw (10,2) node[name=alpharesponsibilitySCBot] {{$\alpharesponsibilitySCBot{}{}{}$}};
     \draw[semithick,dotted, <-] (alpharesponsibilitySC) -- (alpharesponsibilitySCBot) node [midway, above, sloped] (TextNode) {$\bar{\alpha}$};
     \draw[semithick] (botR) -- (alpharesponsibilitySCBot);
     \draw (7,4) node[name=alpharesponsibilitySCH] {{$\alpharesponsibilitySCH{}{}{}$}};
     \draw[semithick, <-] (alpharesponsibilitySCBot) -- (alpharesponsibilitySCH) node [midway, below, sloped] (TextNode) {$\alphaFuture{}$};
     \draw (16,4) node[name=alpharesponsibilitySCF] {{$\alpharesponsibilitySCF{}{}{}$}};
     \draw[semithick, <-] (alpharesponsibilitySCBot) -- (alpharesponsibilitySCF) node [midway, above, sloped] (TextNode) {$\alphaHistory{}$};
     \draw (13,6) node[name=alpharesponsibilitySCTop] {{$\alpharesponsibilitySCTop{}{}{}$}};
     \draw[semithick, <-] (alpharesponsibilitySCH) -- (alpharesponsibilitySCTop)  node [near end, above, sloped] (TextNode) {$\alphaHistory{}$};
     \draw[semithick, <-] (alpharesponsibilitySCF) -- (alpharesponsibilitySCTop) node [midway, above, sloped] (TextNode) {$\alphaFuture{}$};

     \draw (10,7) node[name=alpharesponsibilityCBot] {{$\alpharesponsibilityCBot{}{}{}$}};
     \draw[semithick,dotted, <-] (alpharesponsibilityC) -- (alpharesponsibilityCBot) node [midway, above, sloped] (TextNode) {$\bar{\alpha}$};
     \draw (7,9) node[name=alpharesponsibilityCH] {{$\alpharesponsibilityCH{}{}{}$}};
     \draw[semithick,<-] (alpharesponsibilityCBot) -- (alpharesponsibilityCH);
     \draw (16,9) node[name=alpharesponsibilityCF] {{$\alpharesponsibilityCF{}{}{}$}};
     \draw[semithick,<-] (alpharesponsibilityCBot) -- (alpharesponsibilityCF);
     \draw (13,11) node[name=alpharesponsibilityCTop] {{$\alpharesponsibilityCTop{}{}{}$}};
     \draw[semithick,<-] (alpharesponsibilityCH) -- (alpharesponsibilityCTop);
     \draw[semithick,<-] (alpharesponsibilityCF) -- (alpharesponsibilityCTop);

     \draw[semithick,line width=1pt,<-] (alpharesponsibilitySCBot) -- (alpharesponsibilityCBot);
     \draw[semithick,<-] (alpharesponsibilitySCF) -- (alpharesponsibilityCF) node [midway, above, sloped] (TextNode) {$\alphaSCbar{}$};
     \draw[semithick,<-] (alpharesponsibilitySCH) -- (alpharesponsibilityCH);
     \draw[semithick,line width=0.4pt,<-] (alpharesponsibilitySCTop) -- (alpharesponsibilityCTop);


     \draw (10,12) node[name=alpharesponsibilityBot] {{$\alpharesponsibilityBot{}{}{}$}};
      \draw[semithick,dotted,<-] (alpharesponsibility) -- (alpharesponsibilityBot) node [midway, above, sloped] (TextNode) {$\bar{\alpha}$};
    \draw (7,14) node[name=alpharesponsibilityH] {{$\alpharesponsibilityH{}{}{}$}};
     \draw[semithick,<-] (alpharesponsibilityBot) -- (alpharesponsibilityH);
     \draw (16,14) node[name=alpharesponsibilityF] {{$\alpharesponsibilityF{}{}{}$}};
     \draw[semithick,<-] (alpharesponsibilityBot) -- (alpharesponsibilityF);
     \draw (13,16) node[name=alpharesponsibilityTop] {{$\alpharesponsibilityTop{}{}{}$}};
     \draw[semithick,<-] (alpharesponsibilityH) -- (alpharesponsibilityTop);
    \draw[semithick,<-] (alpharesponsibilityF) -- (alpharesponsibilityTop);

     \draw[semithick,line width=1pt,<-] (alpharesponsibilityCBot) -- (alpharesponsibilityBot);
     \draw[semithick,<-] (alpharesponsibilityCF) -- (alpharesponsibilityF) node [midway, above, sloped] (TextNode) {$\alphaCbar{}$};
     \draw[semithick,<-] (alpharesponsibilityCH) -- (alpharesponsibilityH);
     \draw[semithick,line width=0.4pt,<-] (alpharesponsibilityCTop) -- (alpharesponsibilityTop);

     \draw (13,18) node[name=topR] {{$\top_R$}};
     \draw[semithick] (alpharesponsibilityTop) -- (topR);
\end{tikzpicture}
\vskip-1em
\caption{Lattice of Responsibility Analysis Results Ordered by $\subseteq$}
\label{fig:lattice-definitions}
\vskip-1em
\end{figure}

%\begin{figure}[h]
%\centering
%\includegraphics[width=.33\linewidth]{Figures/lattice-definitions.pdf}
%\caption{Lattice of Responsibility Analysis Results}
%\label{fig:lattice-definitions}
%\end{figure}

Besides from the definitions in the above lattice, there are possibly other useful definition of responsibility via the monitor $\monitor{}{}{}$. For example, the following $\alpharesponsibilityPearl{\monitorsymbol\sqb{\observer}}{\maximalsemantics{}}{}$ is a counterfactual responsibility that ignores the whole history and keeps the further future (i.e. suppose $\tracefuturebar=\tracefuture'\tracefuture''$, instead of keep the whole $\tracefuturebar$ by requiring $\tracefuture=\tracefuturebar$, only the second part $\tracefuture''$ is kept in $\tracefuture$).

\begin{eqntabular}[fl]{@{}L@{}rcl}
% Keep only the future
\rlap{\textit{Counterfactual responsibility with further future.\quad}}\nonumber\\
%%%&\alpharesponsibilityPearl{\monitorsymbol\sqb{\observer}}{\maximalsemantics{}}{} &\in& \wp(\setofalltraces)\mapsto\wp(\setofalltraces\times\setofalltraces\times\setofalltraces\times\wp(\setofalltraces)\times\setofalltraces\times\setofalltraces) \nonumber
%%%\\
&\alpharesponsibilityPearl{\monitorsymbol\sqb{\observer}}{\maximalsemantics{}}{\traceproperty}&\triangleq& \{\sextuple{\tracehistory}{\traceresponsible}{\tracefuture}{\behavior}{\tracehistorybar}{\tracefuturebar}\mid\wedge\tracehistorybar\traceresponsible\tracefuturebar\in\maximalsemantics{}\wedge|\traceresponsible|=1\nonumber
\\
&&&\quad{}\wedge\behavior\in\monitor{}{\observer}{\prefixes{\tracehistorybar\traceresponsible}}\backslash\monitor{}{\observer}{\prefixes{\tracehistorybar}}\wedge\tracehistory\traceresponsible\tracefuture\in\traceproperty\cap\maximalsemantics{} \nonumber
\\
&&&\renumber{${}\wedge\exists\traceresponsible', \tracefuture', \tracefuture''\in\setofalltraces.\;|\traceresponsible'|=1\wedge\tracefuturebar=\tracefuture'\tracefuture''$}
\\
&&&\renumber{${}\wedge\exists\behavior'\in\monitor{}{\observer}{\prefixes{\tracehistorybar\traceresponsible'\tracefuture'}}.\;\behavior\not\sqsubseteq\behavior'\wedge\behavior'\not\sqsubseteq\behavior$}
\\&&&\renumber{$\wedge\exists\tracefuture'''\in\setofalltraces.\;\tracefuture=\tracefuture'''\tracefuture''\}$}
\end{eqntabular}

This definition is more loose than $\alpharesponsibilityCF{\monitorsymbol\sqb{\observer}}{\maximalsemantics{}}{}$ (i.e. $\forall\traceproperty\in\wp(\setofalltraces).\;\alpharesponsibilityCF{\monitorsymbol\sqb{\observer}}{\maximalsemantics{}}{\traceproperty}\subseteq\alpharesponsibilityPearl{\monitorsymbol\sqb{\observer}}{\maximalsemantics{}}{\traceproperty}$). It can deal well with every example in \cite{Halpern-Pearl-2001,Halpern-Pearl-2005}, and we conjecture that it has the same power as actual cause.
